Putting words in context: LSTM language models and lexical ambiguity

In neural network models of language, words are commonly represented using context-invariant representations (word embeddings) which are then put in context in the hidden layers. Since words are often ambiguous, representing the contextually relevant information is not trivial. We investigate how an LSTM language model deals with lexical ambiguity in English, designing a method to probe its hidden representations for lexical and contextual information about words. We find that both types of information are represented to a large extent, but also that there is room for improvement for contextual information.

==> related_work.tex <==
\section{Related work}
\label{sec:relwork}

\gbt{Limit the discussion of related work to the following topics; probably merge with intro.}

\begin{itemize}
\item meaning in context in DS (also compositional DS)
\item contextualized word representations in DL
\item interpretation of DL models; probe tasks
\end{itemize}

% Lexical ambiguity in linguistics and NLP	
%\begin{itemize}
%	\item Linguistics	
%	\item Work in NLP separating different phenomena
%	\item Lexical ambiguity in word embeddings
%	\item Multi-prototype representations
%	\item Contextualized representations of words
%\end{itemize}

%Accounting for how lexical ambiguity is resolved in communication has long posed challenges to researchers in Linguistics and Cognitive Science (see \citealp{falkum2015} for an overview).
Lexical ambiguity has long posed challenges for researchers in NLP, which have been addressed by several perspectives and methods.
%Many approaches provided separate accounts for the different phenomena (e.g., regular polysemy, metaphor); others instead attempted at tracing these back to a general resolution mechanism (e.g., ).
%An analogous pattern can be somewhat found in how lexical ambiguity has been treated in NLP models. 
For instance, a body of research developed models addressing specific phenomena involving variations in a word's meaning (e.g., regular polysemy, metaphor; ... ); another has instead focused on general methods to resolve ambiguity, such as pointing a discrete sense of a word, or obtaining a contextual representation of it. 
Due to the topic of this paper, we here focus on the latter case. 

For most of these methods, the starting point have been vectorial representations of words, constructed on the basis of their use (aka Distributional Semantics).
Though these provide a powerful way to represent words, they are subject to a series of shortcomings.
By associating each word to one representation based on all its uses, (1) they do not steadily provide a way to represent its meaning variation across contexts, and (2) they collapse in one representation information relevant to different of its senses.
%For this reason they are not apt to represent the meaning that a word has in a particular context of use. 
The solution that some found is to learn distinct representation for each sense of a word - \textit{multi-prototype} approaches (...). 
Others methods instead dynamically adapt the word representation to the linguistic context the word is encountered in (...). 
One of the benefits of the last approach is that they go beyond a set of discrete word senses, and can represent the variations of a word's meaning in a nuanced fashion.

%One of the core idea behind these is that
%, even though distributional semantic representations are not representations of a word's specific use, they can act as a gateway for it: 
%since distributional semantic representations encompass information associated to different uses, when re-weighted according to the context, the relevant one is highlighted, leading to represent the contextual nuance.

Yet, only recently, using contextual representations of words as inputs to NLP models have become a common practice. 
This happened after the introduction of a series of methods that derive context-dependent representations using activations of deep learning models.
For example, in the case of ELMo, a representation is obtained as a function of its static embedding and the hidden states of a language model at its timestep.
%These embeddings can be employed as input in whichever model taking words as input, in the place of the static word embeddings: while the weights of the language model used to form the activations are not trained, the way these are combined is fit to the objective task.
%However, 
These representations were shown to capture contextual properties of a word, such as its part of speech, word sense or co-reference chain.
This occurs without disambiguation being an explicit objective of the model from which they were obtained; for example, in the case of ELMo, an LSTM language model.
This provides evidence that the internal representations of this kind of model may already contain sufficient information for discriminating the contextually-relevant meaning of the word. 


%This allows different models to focus on different activations: in practice, this has showed that different hidden layers capture different word information.
%(TOADD: Also they are doing more than disambiguation really ....)


%No explicit and directly interpretable disambiguation step within the processing of models employing static word embeddings as inputs. 
%Yet the latter have been widely successful in several tasks, or to obtain representations that do capture contextual properties of words.
%This suggests that models may learn to implicitly resolve the aforementioned ambiguity present in word embeddings, without the need of ad hoc methods. 


%\texttt{TOADD:Context2vec}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

